Graph Ranking and the Cost of Sybil Defense

Ranking functions such as PageRank assign numeric values (ranks) to nodes of graphs, most notably the web graph. Node rankings are an integral part of Internet search algorithms, since they can be used to order the results of queries. However, these ranking functions are famously subject to attacks by spammers, who modify the web graph in order to give their own pages more rank. We characterize the interplay between rankers and spammers as a game. We define the two critical features of this game, spam resistance and distortion, based on how spammers spam and how rankers protect against spam. We observe that all the ranking functions that are well-studied in the literature, including the original formulation of PageRank, have poor spam resistance, poor distortion, or both. Finally, we study Min-PPR, the form of PageRank used at Google itself, but which has received no (theoretical or empirical) treatment in the literature. We prove that Min-PPR has low distortion and high spam resistance. A secondary benefit is that Min-PPR comes with an explicit cost function on nodes that shows how important they are to the spammer; thus a ranker can focus their spam-detection capacity on these vulnerable nodes. Both Min-PPR and its associated cost function are straightforward to compute.

==> conclusion.tex <==
\section{Conclusion}

\todo{a section putting all our results in context and relation with each other}

==> cover.tex <==
Dear EC PC Committee,
\medskip

We would like to submit our paper, \emph{Graph Ranking and the Cost of Sybil Defense}, to EC.  It was recently rejected from STOC, so we are including the referee reports from that reviewing process.  Those reviews can be summarized in the following points:
\medskip

\begin{itemize}
\item The paper involves formalizing the arms race between graph rankers (e.g.\ Google) and spammers.  The game has various components, including a cost function that codifies how much effort a ranker is putting into detecting the spammer's acquisition of previously valid nodes.  The more the effort, the greater the cost to the spammer of subverting a node.

In addition, the paper uses the formalized spam game to prove results on existing ranking functions (which verify intuition).  Finally, the paper provides positive results for one ranking function and validates those results experimentally. 

\item The reviewers agreed that the results were technically non-trivial and interesting.  The consensus was that this would be a good paper for a more focused conference, hence the submission to EC.

\item One reviewer had a technical question involving the cost function that codifies the interaction between the graph ranker and the spammer---specifically, is this cost function  computable by the ranker?
It is. 
Indeed, one of the main points of the paper is that the proof of spam resistance generates an explicit (computable) cost function.  Ultimately, our result shows that there is an elegant ranking function available to the ranker (independent of the cost function) that reduces the spamming game to an arms race between the ability of the ranker to detect spam nodes and the ability of the spammer to subvert nodes without detection.

\item Finally, one reviewer wondered what the follow-up work would be like for this paper. 
Although we are excited about what we were able to show for graph rank spamming (and we feel that this line of work itself has interesting follow-up), we're even more excited %by the new graph-theoretic problems that these definition open up. 
by the opportunity to use our approach to define spamming games in other situations (e.g.\ Wikipedia spamming, benchmark spamming, H-index spamming, etc.). 
\end{itemize}


We conclude with Goodhart’s Law: ``When a measure becomes a target, it ceases to be a good measure,'' which encapsulates the ubiquity of spamming.  

\medskip

Sincerely,

\bigskip
\bigskip
\bigskip

The anonymous authors


\newpage




\begin{relate}
\item[Review \#89A: ]
\emph{Summary of the main contributions of the paper:}
While prior work on the Sybil attacks on graph ranking functions either treats it heuristically or focuses on specific functions versus specific attacks, this paper proposes two features to enable the theoretical study of to what extent PageRank functions are resistant to Sybil attacks. Specifically, the first feature, spam resistance, utilizes the cost/benefit ratio caused by the Sybil attack to see how much the functions are resistant. The second feature, distortion, compares the function values with stationary distributions of uniform random work on web graphs to see how the function results are distorted from it. 
After showing PageRank functions that are classic in the literature either have poor spam resistance, poor distortion, or both, it shows that Min-PPR, the ranking function used in Google, has both good spam resistance and good distortion on graphs with worst-case and average-case fast mixing time, respectively. 
\smallskip

\emph{What is best about the paper:}
What I like about this paper is that it proposes two general features, one to measure the ability of an arbitrary ranking function to reveal the importance of nodes, and the other one to its resistance to Sybil attacks. With the analysis of classic examples, the insights of the two main theorems are well-delivered to me. Also, the closure property of the PageRank function class under component min operation may be applied to other problems, and the idea may be used to find out more operations and functions with good properties. 
\smallskip

\emph{What are the paper's weaknesses:}
My main concerns are about the practical applicability of the cost functions, when defining the spam resistance, and the selection of centers in the main theorem of Min-PPR's good distortion:
1. The cost function of acquiring nodes by a spammer is a function of the whole true graph $G$. However, the ranker should not know what the true graph is and therefore fail to compute the true value of the function. Therefore, in my understanding, the cost function should not be applicable in practice, but only a quantitive measure, used in defining the spam resistance, of how important a node is to defend a ranking function from the Sybil attack. 2. In the main theorems on T-Min-PPR's good distortion property, $K$ centers are chosen according to the distribution, defined by the PageRank result of arbitrary reset vectors, while the definition of T-Min-PPR requires that the centers are chosen only in trusted nodes and has nothing to do with the whole graph. The authors should mention that, for arbitrary graphs and the set of trusted nodes, if there exists a reset vector, such that, the corresponding PageRank distribution only put mass on trusted nodes, so that the results will apply to the T-Min-PPR function. 
\smallskip

\emph{The paper's target audience:}
This paper is readable to the audience with basic knowledge of Markov chains and PageRank.
\medskip

\item[Review \#89B:] 

\emph{Comments for author:}
The paper studies sybil attacks on PageRank and related web ranking algorithms. In the web ranking problem, the input is a directed graph, where nodes represent web pages and edges are web links. The output is an assignment of non-negative values to the vertices summing to one. A higher value corresponds to a higher importance/rank. The PageRank algorithm solves this problem by assigning to each node its probability in the stationary distribution in a random walk, where with probability eps the next node is uniformly random, and with probability 1-eps it is a uniformly random outgoing neighbor. 
In the problem under consideration, there is an adversary (a spammer) who tries to increase the rank of a set of nodes that it controls. The adversary can create arbitrarily many nodes and links from a node it owns to any other node in the graph. This captures the fact that a spammer can create many fake websites and links from them. Pagerank is not robust against such an adversary: the spammer can simply create a large clique and essentially capture all rank.
\small skip

To address the above limitation, the paper proposes a refinement of the model where there are some trusted nodes that the adversary cannot corrupt. A modified version of PageRank is studied, called Min-PPR. In this algorith, k different rankings are computed, where in each one the random walk restarts at some fixed node c, with probability eps (instead of a uniformly random node, as in PageRank). Then, the final weight of a node is the minimum of the k stationary probabilities (normalized so that the sum of all weights equals 1). Interestingly, Min-PPR, is essentially an algorithm that Google itself used to fight spam in web ranking, according to a personal communication with an early Google employee.
\smallskip

The main contribution of the paper is in showing that Min-PPR is robust against sybil attacks, while approximately preserving the original ranking (i.e. without an adversary), for graphs with good mixing times. To that end, the paper defines an interesting notion of "distortion" of a ranking, which, roughly speaking, ignores nodes with rank below some polynomial threshold. The condition on the mixing time seems necessary. It is also realistic since the web graph seems to enjoy this property.
\smallskip

The paper is very well written. The technical part is quite non-trivial.
\smallskip

In summary, I think this is a fairly interesting conceptual contribution. My main hesitation for recommending acceptance to STOC is that the problem studied in this paper does not seem of wide enough interest currently. The sybil resistance of PageRank was an important problem several years ago. However, it seems unlikely that the results presented here will help design better ranking algorithms, since the problem seems already solved in practice. Moreover, modern day web ranking probably involves many more factors that are not captured here. Finally, even though the model is conceptually interesting, I don't foresee any new research direction coming out of this work.
\medskip

\item[Review \#89C:]
\emph{Comments for author}
This paper investigates ranking functions for the web graph regarding their protection against spamming. A ranking function assigns a numerical value (between 0 and 1) to each node; it can be seen as a probability distribution over nodes. 
The authors formalize mathematically two criteria: spam resistance and distortion. They investigate well-studied ranking functions from the literature (including the original formulation of PageRank) and observe that they have behave poorly with respect to one or both criteria.
\smallskip

They study then the a variant of PageRank called Minimum Personalized PageRank, Min-PPR, (which they claim google is using) and show that it is highly spam resistant and has low distortion. This ranking function has not been treated in the literature.
\smallskip

The main technical contribution is (a) the formal definition of the criteria and (b) the  investigation of ranking functions based on the analysis of random walks and mixing times. 
The strength of the paper is that it provides interesting definitions and analyses of different ranking functions. Defining proper criteria is clearly a non-trivial task, but I find it difficult to judge how well the proposed measures capture the desired properties. To me, the importance and relevance of the proven bounds remain still unclear. I wished the authors would have helped me with some more interpretation. (Maybe it is targeted at a more specialized audience as also the literature list suggests.) On the technical side, the analysis appears non-trivial but does not need heavy machinery and does not introduce new methods.

\end{relate}

==> intro-previous.tex <==
%!TEX root = ./paper.tex

\newpage

\section{Introduction}\label{sec:intro}

% \john{Proposed replacement for intro, post-merging the old intro.}

%Ranking functions such as \pr~\cite{DBLP:journals/cn/BrinP98} that assign numeric values (\emph{ranks}) to nodes of the web graph are an integral part of Internet search algorithms, since they can be used to order the results of queries. 

Ranking functions such as \pr~\cite{DBLP:journals/cn/BrinP98} assign numeric values (\emph{ranks}) to nodes of graphs, most notably the web graph.  Node rankings are an integral part of Internet search algorithms, since they can be used to order the results of queries. 
However, these ranking functions are famously subject to attacks by spammers, who modify the web graph in order to give their own pages more rank. 

In the literature on ranking functions, resistance to spam attacks is treated heuristically~\cite{fogaras2005towards,gyongyi2004combating,liu2016personalized,Ng:2001:SAL:383952.384003} 
%\mfc{split citation list} 
or with respect to specific ranking functions versus specific attacks~\cite{cheng2006manipulability,hopcroft2008manipulation,DBLP:conf/ijcai/NgZJ01}.
Much of the ranking literature has focused on two aspects of fighting spam: link-spam detection~\cite{gyongyi2006link,cheng2006manipulability,DBLP:conf/airweb/AndersenBCHJMT08,DBLP:journals/ton/YuGKX10,yu2008sybilguard,Yu:2011:SDV:2034575.2034593,alvisi2014communities}; and heuristically designing ranking functions that are spam resistant~\cite{kumar2006core, bhattacharjee2006incentive, gyongyi2004combating,gyongyi2004combating,krishnan2006web,hopcroft2008manipulation,liu2016personalized}.


%In this paper, we begin by showing how to bound the vulnerabilities of arbitrary  ranking functions against the class of all possible spam attacks, e.g., the spammability of novel ranking functions against which no attacks have yet been mounted in the real world, the vulnerabilities of existing ranking functions against previously unseen attacks, etc.  We complement this formalization with results on specific ranking functions: we show that the well-known ranking functions offer poor performance against spam attacks but show that there is a ranking function that is highly spam resistant.


We combine the notion of attack detection and attack resistance into a single two-party game that allows us to reason about ranking functions.
\begin{itemize}[noitemsep,nolistsep]
\item A spammer can perform a \emph{Sybil attack}\footnote{The moves by the spammer are quite general and subsume specific attacks treated in the literature~\cite{viswanath2011analysis}}:
\begin{itemize}[noitemsep,nolistsep]
	\item Create as many nodes in the web graph as they like, for free;
	\item Change the out-links of all nodes they own, for free;
	\item Acquire (by buying, hacking, etc) existing nodes in the web graph, at some cost, except for nodes in a non-empty \emph{trusted set}, which cannot be acquired.
\end{itemize}


\item The ranker can: \begin{itemize}[noitemsep,nolistsep]
	\item Modify the ranking function to make it more resistant to spam, subject to quality constraints;%, which we characterize below as low \textit{distortion};
    \item Expend effort to detect if nodes have been acquired by spammers, which we model as raising the cost for spammers to acquire those nodes.
\end{itemize}
\end{itemize}
In this game, the spammer wants to maximize the sum of rank of its nodes, and naturally the ranker wants to minimize this quantity.  The spammer knows the ranking function and the cost function, whereas the ranker does not know what actions the spammer is taking.


%Detecting (and removing) Sybil attacks is the focus of much of the literature in this area~\cite{fillin}, but in this paper, we will consider the interplay between spam resistance and spam detection, which allows us to bound the payoff that a spammer can achieve.
Trusted nodes play a critical role.
Without trusted nodes, the ranker cannot hope to resist a spam attack, because the spamming model is general enough that  the spammer could make a complete (or partial) replica of the web  graph, and the ranker would not know which is the correct version.  On the other hand, the ranker cannot simply rank trusted nodes and ignore untrusted nodes because: it is prohibitively expensive to certify that all unspammed nodes are trusted; and, restricting rank to only a few nodes would introduce local (ranking-function) \emph{distortions},  formally defined in Section~\ref{sec:def-distortion}.


This rather broad characterization of spam attacks and defense leaves two obvious questions:
\begin{itemize}[noitemsep,nolistsep]
	\item Is there a way to define the spam resistance and distortion of arbitrary ranking functions that is mathematically tractable and matches intuition and practice?
	\item Do these definitions yield mathematical and practical insight?  That is, can we prove that there is a ranking function with both low distortion and high spam resistance? In other words, does the ranker have a good strategy?  
\end{itemize}

\pp{Our contribution.} In this paper, we answer both questions in the affirmative. In Section~\ref{sec:def-spam-resistance}, we show that the simple rules above are enough to define spam resistance as the highest cost-benefit ratio the ranker can force on the spammer.  We survey what is known about common ranking functions and demonstrate that our definition matches intuition and practice. We show that any ranking function that does not make use of a trusted set offers no spam resistance. This includes the original definition of \pr and many other common ranking functions.


In our survey of ranking functions, we find that the rankers that are most spam-resistant, e.g. a function that assigns non-zero rank only to trusted sites, introduce unacceptable local distortion.
In Section~\ref{sec:def-distortion}, we formalize this notion of distortion in a way that captures intuition about many real-world ranking functions. We do so by considering Brin and Page's original motivation for defining \pr~\cite{page1999pagerank}: that in the case of a graph with an ergodic random walk, the correct ranking function would be the stationary distribution of this random walk. In fact, in the absence of spam, in an axiomatic sense this stationary distribution and \pr, itself, are the only natural ranking functions~\cite{axioms_pagerank}. 
We say that a ranking function $f$ has low distortion if, in the absence of spam, $f$ agrees very closely with the stationary distribution on all sites with any significant weight in this distribution.  Although the quality of a ranking function may depend on many factors that are beyond the scope of this paper, we find that there is an intuitive tradeoff between spam resistance and distortion in that we observe, rather dispiritingly, that all ranking functions in the literature exhibit either high distortion, low spam resistance, or both.

Interestingly, this leaves open the question of the properties of the type of \pr that Google itself used.  To the best of our knowledge, Google has never used uniform reset \pr for web-search ranking, in part because of its obvious susceptibility to spammers.  Instead, Google has used a variant of \pr that we call Min-PPR (and which we define below), because it was intuitively considered to be more spam resistant~\cite{MFC}.  We know of no treatment of Min-PPR in the literature.



In Section~\ref{sec:results}, we set out our main 
contribution: we show that this faith in Min-PPR is well placed.  We prove that Min-PPR exhibits both low distortion and high spam resistance subject to the mild technical condition of fast mixing. Fast mixing is known to hold in real-world social and semantic networks, and if it does not hold then we prove that no variant of \pr has low distortion. No ranking function is spam resistant if the ranker makes no effort to detect spam, so we also show that we can compute a cost function for Min-PPR that 
establishes the importance of each node in fighting spam.  In other words, this cost function shows which nodes the ranker should focus its spam-fighting efforts on.

Proving these results requires a substantial technical contribution: while our definitions of distortion and spam resistance are natural, they are also difficult to analyze. The proof that establishes the distortion of Min-PPR relies on a sophisticated analysis of mixing times (see Section~\ref{sec:distortion}), whereas the proof that establishes the spam resistance of Min-PPR relies on a intricate extremal argument (see Section~\ref{sec:termispam}). 


Min-PPR is based on a variant of \pr known as Personalized \pr, which is intended to give a personalized ranking of sites relative to a center node~\cite{DBLP:conf/www/JehW03}. We prove that Personalized \pr is highly spam resistant if the center node is trusted, but also has high distortion. % (as one might expect given its purpose). 
This distortion comes in the form of a ``spike'' of abnormally high rank around the center node, which we show can be almost totally ameliorated by taking the component-wise minimum of multiple PPRs with distinct center nodes. Not every choice of centers has this property, but we prove that almost every choice does. 
%As an aside, we include an experimental validation of our theoretical results in Appendix~\ref{sec:appendix}.

Along the way we also prove some other results that may be of independent interest, also stated in Section~\ref{sec:results}. These include: a variant of our bound on the distortion of Min-PPR which requires only a substantially weaker condition on mixing time; the fact that all \prs with suitably low reset probability are close in total variation distance; 
and that \prs exhibit two forms of closure. 
We show that Min-PPR is itself a \pr via \emph{strong} closure, whereas  Median-PPR is only a \pr under \emph{weak} closure, defined below.

In this paper, we reimagine the arms race between web rankers and web spammers as a two-person game.  We define the moves of each party.  We show that there is a natural tension between spam resistance and distortion, but we show that the ranker can gain the upper hand; that is, we exhibit a ranking function that has low distortion and high spam resistance.  
%This formalism sets up web spamming for a more complete game-theoretic treatment, which we leave for future work.



\pp{Roadmap.} In Section~\ref{sec:prelim}, we introduce preliminary notation.  In Section~\ref{sec:def-spam-resistance}, we formally define spam resistance and in Section~\ref{sec:def-distortion}, we formally define distortion.  In both sections, we survey existing ranking functions and provide preliminary results.  In Section~\ref{sec:results}, we formally define Min-PPR and give an overview of the main theorems related to its spam resistance and distortion.  In Section~\ref{sec:closure}, we explore the algebraic properties of \pr, including its closure structure.  In Sections~\ref{sec:distortion} and~\ref{sec:termispam}, we prove the theorems outlined in Section~\ref{sec:results}.  In Section~\ref{sec:related}, we discuss related work. In Appendix~\ref{sec:appendix}, we present experimental results.



%These closure properties provide a natural motivation for considering Min-PPR over, for example, Median-PPR.

%The full proofs of all claims can be found in the attached appendix.



% \john{End of proposed replacement.}

% \bigskip
% \hrule
% \bigskip

% \john{Old stuff.}

% % \john{Possible snappier alternative to first two paragraphs.}

% Ranking functions such as \pr~\cite{DBLP:journals/cn/BrinP98} that assign numeric values (\emph{ranks}) to nodes of the web graph are an integral part of Internet search algorithms, since they can be used to order the results of queries. 
% However, these ranking functions are subject to attacks by spammers, who modify the web graph in order to attempt to give their own pages more rank. 


% \mfc{TO MERGE with target below?
% In the literature on ranking functions, resistance to spam attacks is talked about intuitively or with respect to specific attacks; local inaccuracy (which we call distortion) is bundled into general discussions of ranking quality, and typically evaluated by numerical experimentation and statistical analysis on specific example graphs. One of our main contributions is to formalize these notions by defining spam resistance and distortion in ways that capture the intuition of many real-world examples, as detailed in Sections \ref{sec:def-spam-resistance} and \ref{sec:def-distortion}. This makes it possible to systematically evaluate the distortion and spam resistance of classes of ranking~functions.}\john{I think the first half of this paragraph should be merged with the second paragraph of the intro, it reads stronger.}

% \mfc{Again, to merge with target below?
% Although there is an extensive literature on characterizing particular spam attacks against particular versions of \pr~\cite{hopcroft2008manipulation,liu2016personalized,cheng2006manipulability,fogaras2005towards,gyongyi2004combating,Ng:2001:SAL:383952.384003,DBLP:conf/ijcai/NgZJ01}, this does not help us understand the vulnerabilities of a new proposed ranking function, one for which no attacks have been mounted in the real world.  To study new ranking functions, we need to characterize the general notion of a spam attack. We therefore introduce a model that is general enough to capture any spam attack} \john{Again, some of these points would fit nicely in the second paragraph of the new intro, and maybe also the big list of citations.}

% \mfc{target of merge?} Such spam attacks come in many varieties, as described in Section~\ref{sec:related}, but we can characterize the class of all possible attacks by observing which changes the spammer is free to make and which changes the ranker is free to make.  A common-sense analysis of the web gives the following operations and their costs:

% A spammer can:
% \begin{itemize}[noitemsep,nolistsep]
% 	\item Create as many nodes in the web graph as they like, for free;
% 	\item Change the out-links of all nodes they own, for free;
% 	\item Acquire existing nodes in the web graph, at some cost in money or effort, except for nodes in a non-empty \emph{trusted set}, which cannot be acquired.
% \end{itemize}

% Naturally, the ranker would like to minimize the amount of rank a spammer receives.  The ranker can do this by: 
% % \begin{itemize}[noitemsep,nolistsep]
% % 	\item Modifying the ranking function to make it more resistant to spam, subject to quality constraints (which we characterize below as low \textit{distortion});
% % 	\item Expending effort to detect if nodes have been acquired by the spammer.
% % \end{itemize}

% % -------

% % \john{Possible snappier alternative to the rest.}

% \begin{itemize}[noitemsep,nolistsep]
% 	\item Modifying the ranking function to make it more resistant to spam, subject to quality constraints (which we characterize below as low \textit{distortion});
%     \item Expending effort to detect if nodes have been acquired by spammers, thereby raising the cost for spammers to acquire those nodes.
% \end{itemize}

% Note the ranker cannot simply restrict non-zero rank to trusted nodes because, on the one hand, it would be prohibitively expensive to certify that all unspammed nodes are trusted if they are many, and on the other, restricting non-zero rank to only a few nodes would make the distortion very high.


% % \john{I think the point of the next two paragraphs is already made clear by the above two bullets, at least to the extent they can be without hard definitions, so let's skip them.}

% This rather broad characterization of spam attacks and defense leaves two obvious questions:
% \begin{itemize}[noitemsep,nolistsep]
% 	\item Is there a way to define the spam resistance and distortion of arbitrary ranking functions that is mathematically tractable and matches intuition and practice?
% 	% "To an arbitrary attack" is already implicit in the above framework, I think.
% 	\item Is there a ranking function with both low distortion and high spam resistance? In other words, does the ranker have a good strategy?  
% \end{itemize}

% \pp{Contribution.} In this paper, we answer both questions in the affirmative. We show that the simple rules above are enough to define spam resistance as the highest cost-benefit ratio the ranker can force on the spammer by setting spamming costs on nodes. We show that any ranking function, including the original definition of \pr and many other common ranking functions, that does not make use of a trusted set offers no spam resistance since it is susceptible to attacks by making new nodes.
% % We show that many common ranking functions offer no spam resistance because they either depend on the out-edges of a node or are susceptible to attacks by making new nodes. 

% % \john{Instead of this sentence I suggest: ``We show that any ranking function, including the original definition of \pr and many other common ranking functions, that does not make use of a trusted set offers no spam resistance since it is susceptible to attacks by making new nodes.'' Advantages: justifies the presence of the trusted set; immediately tells referees who are thinking ``but what about specific approach/paper X?'' that most likely X does not work; I don't think we prove anything has zero spam resistance because it depends on the out-edges of a node?}

% In defining distortion, we first consider Brin and Page's original motivation for defining \pr~\cite{page1999pagerank}: to create a natural measure that is defined on all graphs, and that would approximate the stationary distribution of a random walk on graphs with an ergodic random walk. In fact, in the absence of spam, in an axiomatic sense this stationary distribution and \pr are the only natural ranking functions~\cite{axioms_pagerank}. Loosely speaking, we say a ranking function $f$ has low distortion if, in the absence of spam, $f$ agrees very closely with the stationary distribution on all sites with any significant weight in this distribution. We show that many common ranking functions, including the original definition of \pr, have high distortion.

% % For distortion, we consider Brin and Page's original motivation for defining \pr~\cite{page1999pagerank}.  They defined \pr in order to approximate the stationary distribution of a random walk, but to be defined on all graphs. We find that considering the relative error of a ranking function with respect to this stationary distribution strongly captures the intuitive notion of distortion.  Many common ranking functions also have high distortion.

% % \john{Instead of this paragraph I suggest:

% % In defining distortion, we first consider Brin and Page's original motivation for defining \pr~\cite{page1999pagerank}: to create a natural measure that is defined on all graphs, and that would approximate the stationary distribution of a random walk on graphs with an ergodic random walk. In fact, in the absence of spam, in an axiomatic sense this stationary distribution and \pr are the only natural ranking functions~\cite{axioms_pagerank}. Loosely speaking, we say a ranking function $f$ has low distortion if, in the absence of spam, $f$ agrees very closely with the stationary distribution on all sites with any significant weight in this distribution. We show that many common ranking functions, including the original definition of \pr, have high distortion.

% % Advantages: \cite{axioms_pagerank} is quite strong for us and we should mention it here; includes a slightly more detailed summary of what distortion is; mentions UPR having high distortion explicitly; a little more detail on what Brin and Page wanted.}

% We are left with the rather dispiriting result that all known ranking functions, including the original definition of \pr, exhibit either high distortion, low spam resistance, or both. Our final contribution is a new variant of \pr, Min-PPR, which we prove exhibits both low distortion and high spam resistance, subject to the mild technical condition of rapid mixing. Rapid mixing is known to hold in (the giant component of) real-world social and semantic networks, and if it does not hold then we argue that no variant of \pr has low distortion.

% % We are left with the rather dispiriting result that ranking functions such as \pr (under the standard definition) have high distortion and low spam resistance.  Our last contribution is exhibiting a \pr variant that has low distortion and high spam resistance.  We next introduce \pr and describe Min-PPR, this new ranking function.  

% % \john{I suggest: 

% % We are left with the rather dispiriting result that all known ranking functions, including the original definition of \pr, exhibit either high distortion, low spam resistance, or both. Our final contribution is a new variant of \pr, Min-PPR, which we prove exhibits both low distortion and high spam resistance, subject to the mild technical condition of rapid mixing. Rapid mixing is known to hold in real-world social and semantic networks, and if it does not hold then we argue that no variant of \pr has low distortion.

% % Advantages: I think we really need to mention the rapid mixing requirement up front; it's not true that every ranking function has both high distortion and low spam resistance, there are plenty which exhibit only one of the two.}

% ===== old stuff below =====


% % \mfc{My proposal for reset of intro.  Move some of this next paragraph to the distortion section, fix up the notation for anythign that refers to it, and mostly just shorten and clean up.}

% % \mfc{and of course clean out anythign taht's already mentioned}

% % \mfc{also, we should figure out which citations and bits of text to move up.}

% % \miguel{The story has been told. I think here we can open a new section Preliminaries with the stuff that follows (whatever is not redundant and needed to spell out the results more formally), followed by the Related Work section, and followed by a Results section containing the results subsection below.}

% % \john{I think we should go intro, then related work (since this doesn't rely on our technical definitions), then preliminaries, then the spam resistance, distortion, and results sections exactly as they are now. I don't think it's a good idea to migrate the contents of the spam resistance and distortion sections into a preliminaries section, partly because that's a lot of work in a very short time, and partly because there's a lot of good stuff in there. (Maybe a few small definitions should move to Preliminaries, like the definition of a ranking vector, but not much.) I agree with Martin that the old intro should now be cannibalised into the Preliminaries section and/or moved up into the new intro. I've gone through and added proposals for what to do with each paragraph.}

% %In the second part of this paper, we discuss our other main contribution --- a new \pr algorithm with higher spam resistance and lower distortion than \UPR, and indeed, with a better combination of these traits than all the main ranking functions, and indeed, than any ranking function we were able to find. These results are stated formally in Section 4 and proved in Sections 5--7.  Our guarantees of high spam resistance and low distortion rely on fast mixing of the underlying ``pre-spammed'' web graph. For this reason, our proofs require a careful analysis of the evolution of the PageRank random walk. \john{This can go. (We do need to add forward references to other sections in the intro though.)}



% % Our model is as follows. Given a graph $\graph{G} = (\nodes,\edges)$, which we think of as the web graph, a spammer can perform the following operations:
% % \begin{itemize}[noitemsep,nolistsep]
% % 	\item Create as many nodes as they like, for free;
% % 	\item Change the out-links of all nodes they own, for free;
% % 	\item Acquire existing nodes in $\nodes$, at some cost in money or effort, except for nodes in a non-empty \emph{trusted set} $\trust$ which cannot be acquired.
% % \end{itemize}
% % \john{This can go, except that we need to make sure the notation $\trust$ gets introduced somewhere.}
% %\john{Slight modifications here as mentioned in email. I think this gets the point across that our core assumptions are sensible and have appeared elsewhere in the literature, but that the Sybil detection people are doing something very different to us and haven't already defined spam resistance.}
% Similar core assumptions are often used informally to analyse Sybil detection algorithms~\cite{viswanath2011analysis}, which are concerned with detecting nodes created by the spammer. In our setting, however, we would like our ranking functions to have the property that the spammer cannot give their nodes high total rank without spending a lot of money or effort. We capture this cost-benefit trade-off by formally defining \emph{spam resistance} in Section~\ref{sec:def-spam-resistance}. For UPR, for example, an attack can be as simple as creating new web pages. This is effectively free, so UPR is trivial to spam, as is well-known in practice~\cite{DBLP:conf/airweb/Baeza-YatesCL05,DBLP:conf/vldb/GyongyiG05}. In fact, we will see that any ranking function that does not make use of trusted vertices is trivial to spam (see Observation~\ref{obs:trust-needed}).
% \john{The points about a similar model being used for Sybil detection algorithms, and UPR's spammability being well-known in practice, are both good and should be ported over.}



% Note that, in the worst case, \UPR can have high distortion. Indeed, for any $\graph{G} \in \ergodicG$, $v \in \nodes$, and $(u,v) \in \edges$, replacing $(u,v)$ with a suitably large collection of internally vertex-disjoint two-edge paths from $u$ to $v$ inflates $\station{\graph{G},\uniform,\rp}[v]$ to a near-arbitrary extent while leaving $\station{\graph{G}}[v]$ almost unchanged (see Observation~\ref{obs:UPR-bad}). 
% \john{This should move to the very end of Section~\ref{sec:def-distortion} (which currently references the introduction).}
% % I don't think "everything gets reset at least \rp/n" is super-persuasive, since you could easily call this an insignificant error. But the construction is good, and we currently reference it in Section 3 without having set it out in the intro. So let's use that instead.


% % Now we talk about PPR in relation to spam resistance at the start, we don't have to set up this part so much.
% Suppose that $c\in\trust$, so that the spammer cannot acquire it. Then in order to obtain high rank, the spammer must expend money or effort to acquire nodes that already have high rank --- it is not enough to simply add new vertices to the graph. So intuitively, \PPR seems less spammable than \UPR.
% % We now talk about UPR having high distortion in the distortion section. It fits much better there, since for our story here we should really be saying "PPR has unacceptably high distortion, which we can fix with Min-PPR" rather than "PPR's distortion is comparable to UPR".
% Unfortunately, this spam resistance comes at a cost. Again intuitively, while \UPR may have high distortion in the worst case, \PPR has high distortion in most cases, since it assigns a rank of at least $\rp$ to its chosen center, and for most centers, this will be far too high.
% \john{This can go, but we should move the intuitive discussion of PPR's spam resistance to the start of Section~\ref{sec:def-spam-resistance} (since it calls back to this).}

% % "while preserving its spam resistance" is important, or it would be easier.
% Can we fix the high distortion of \PPR while preserving its spam resistance?  
% % Adding a more explicit setup for the low-contraction theorem later.
% We would expect the distortion of \PPR with center $c$ to take the form of a ``spike'' in rank at $c$ and nearby vertices, with vertices far from $c$ receiving a \pr which is a little too low but otherwise reasonable. 
% % Some rephrasing here, in particular I don't like ``neighbourhood'' since that's a technical term and the bias could go further than that.
% Suppose we compute two \PPRs with centers $c_1$ and $c_2$ which are distant from each other. Then in $\station{\graph{G},c_1,\rp}$, $c_2$ and nearby vertices will receive an accurate ranking, and in $\station{\graph{G},c_2,\rp}$, $c_1$ and nearby vertices will receive an accurate ranking. The component-wise minimum of $\station{\graph{G},c_1,\rp}$ and $\station{\graph{G},c_2,\rp}$ should therefore yield an accurate ranking for all vertices. 
% \john{This is good stuff, but it no longer fits in the intro, and doesn't seem right for a Preliminaries section either since it heavily relies on intuition we've already built up (that is now being axed). I think it needs to move all the way to Section~\ref{sec:results} where we define Min-PPR.} \john{Actually, I think what's in the intro now covers this already, so it can delete.}



% \textbf{Min versus Median.} It is natural to ask whether, instead of taking the normalized component-wise minimum of our PPRs, we could take the normalized component-wise median. We show that Min-PPR has a crucial advantage over Median-PPR: The normalized minimum of any set of PageRanks with reset probability $\rp$ is itself a PageRank with reset probability $\rp$, whereas the normalized median of any set of \prs with reset probability $\rp$ is a \pr with possibly much larger $\rp$.  

% This preservation of $\rp$ is important, as without it the closure condition would be so weak as to be useless. Notice that, as the reset probability is allowed to become arbitrarily large, the resulting PageRank will approach the reset vector, with little contribution from the underlying graph --- indeed, we show that any strictly positive vector whose entries sum to $1$ is a PageRank.

% We make a distinction between operators that are \emph{strongly closed}, which means they preserve the reset probability, and those that are \emph{weakly closed}, which means that they might not, and show that min is strongly closed for \pr, whereas median is only weakly closed. Indeed, the reset probability of Median-PPR may be as high as 1/2 even when $\rp$ is arbitrarily small.
% \john{...OK, this actually hurts a bit. I think all of this needs to go into Section~\ref{sec:results}, into a little section before the summary called \textbf{Why not median?}. I don't like overloading that section, but I don't see another easy way. Also make sure it's mentioned in the last one or two paragraphs of the contributions section in the intro.}

% % \pp{Min and Median.}
% % It is natural to ask if we should use Median-PPR instead of Min-PPR.  We show that, given $k$ \prs, their normalized component-wise min is a \pr, but we also show that their normalized component-wise median is a \pr, so why choose Min-PPR over Median-PPR?  We introduce two types of closure for \pr, \emph{weak} and \emph{strong closure} for \pr.  A function $f$ is \emph{strongly closed} for \pr if, given $k$ \prs that all use the same $\rp$, the normalized component-wise application of $f$ yields a \pr with the same $\rp$.  It is \emph{weakly closed} if the resulting \pr might require a large $\rp$.  

% % We prove that min is strongly closed for \pr whereas median is only weakly closed.  To see why this matters, notice that as $\rp$ approaches $1$, the resulting \pr approaches the reset vector, which little contribution from the underlying graph. We show that the median of $k$ \prs with arbitrarily small $\rp$ can have an $\rp$ over $1/2$.

% % Reorganised things a bit so that the bullet-point list of results only contains results.
% \pp{Results.} In Section~\ref{sec:def-spam-resistance}, we formally define spam resistance and discuss the spam resistance of UPR and PPR. In Section~\ref{sec:def-distortion}, we formally define distortion and discuss the distortion of UPR and PPR. 
% % I think we need to mention this restriction even in the intro, or the reader will think our results apply to all graphs.
% We also set out a mild condition on the ``pre-spam'' graph (namely fast mixing) without which we cannot expect any PageRank to have low distortion. 
% % "Main technical results" is a flag for SODA referees.
% Subject to this requirement, in Section~\ref{sec:results}, we formally define Min-PPR and state our main technical results: \john{When we add a flag forward to Section~\ref{sec:results} to the intro, I think we do need to mention this is where the technical meat is.}
% % \leslie{Add thm refs. PUt in same order as paper}
% % The stuff in the list is the stuff important to the story. I don't want to list the other Theorems point-by-point, since there's so many of them and the reader will get there eventually...
% \begin{itemize}[noitemsep,nolistsep]
%     \item ``Most'' trusted sets result in dramatically lower worst-case distortion for Min-PPR than is achieved for PPR or UPR (Theorem~\ref{thm:minppr-dist}). More formally, for any graph~$\graph{G}$, if we   choose a set~$\centers$ of $\Omega(\log n)$ centers independently from \emph{any} PageRank on~$\graph{G}$ with any
%     reset vector~$\vect{r}$ and any reset probability~$\rp$
%     then,  
%     with high probability, Min-PPR with  centers~$\centers$ and reset probability~$\rp$ has very low distortion ---
%     the distortion only exceeds the perfect distortion of~$1$ by
%     an additive amount which is of the   order of $\rp \log(|\nodes_{\graph{G}}|)$ times the mixing time of~$\graph{G}$ (often this additive amount is $o(1)$). By contrast, as we will see in Section~\ref{sec:def-distortion}, there are many graphs~$G$ for which UPR and PPR have very high distortion. \john{We no longer need this level of detail in the intro, what's there is fine as long as we add a forward reference to the theorem statement.}
    
   
    
     
     
%     \item Despite this, Min-PPR is almost as spam resistant as PPR; if Min-PPR makes use of $k$ centers, then its spam resistance is within a factor of roughly $3k$ of PPR's spam resistance  (Theorem~\ref{thm:min-spam-resistant} and Observation~\ref{obs:Thm3istight}).
%     By contrast, as we will see in Section~\ref{sec:def-spam-resistance} (see Observation~\ref{obs:trust-needed}), UPR has zero spam resistance on all graphs. \john{Ditto. It's irritating, though, that we can't say ``spam resistance very close to PPR'' any more --- that sounded much stronger. It's even more irritating that Observation~\ref{obs:PPR-bad} could be fairly easily reformulated to work with any PageRank, which we could easily cite (but this would be technical work too close to a deadline) or we could cite the same result from reference B (but they don't quite use our framework so it would be a pain). Not sure what to do about this.}
    
     
% \end{itemize}
% % I think all the stuff that was in the spam resistance paragraph is no longer relevant. We now talk more explicitly about how we define spam resistance in the spam resistance \pp, and we no longer use the reset vector of \minppr to prove spam resistance. And I think the distortion stuff should hopefully sell itself now?
% % We emphasize that our distortion result is a worst-case bound over (fast-mixing) pre-spam graphs. Thus we prove that Min-PPR has the potential to give a far more accurate ranking than even \UPR, while retaining most of the spam resistance of \PPR.

% Along the way we also prove some other results that may be of independent interest, including: a variant of our distortion bound which (by choosing a subset of the trusted set of centers) requires only a substantially weaker condition on mixing time; the fact that all PageRanks with suitably low reset probability are close in total variation distance, rendering total variation distance unsuitable as a distortion; and some new algebraic properties of \prs, including the closure properties mentioned above.\john{This should definitely be ported over to the intro, as a slightly-tweaked final paragraph of the contributions section. Also talk a bit about the intuition of Min-PPR.}

% The full proofs of all claims can be found in the attached appendix.
% \john{This should also be ported over.}

% \john{End of old stuff.}

% \bigskip\hrule\bigskip

% % \leslie{All pageranks close in dtv.
% % Expected-mixing stuff.}

% % some new algebraic properties of \prs, including the closure properties of \pr, mentioned above. 


% % % and a formalization of the idea that PageRank bias comes in the form of positive ``spikes'' introduced by the reset vector.

% % \john{Leslie and I did spend most of our time talking about Theorem 30 yesterday, but we also talked a bit about the intro. We think the proofs in this paper aren't really a selling point for us - they're non-trivial, but they're not bringing anything new to the table in terms of methodology, and they're not \emph{that} difficult by mathsy standards. Our biggest selling point is our results, which are genuinely new and awesome. That's not a problem - you can definitely get into the top conferences with awesome results whose proofs aren't too difficult. Our biggest danger is that some referees think we probably don't have any interesting results because we spend so much time talking about definitions first, which is unusual, and decide to reject us prematurely on that basis. So in our opinion the best way to improve selling in the intro is not to hype the proofs themselves, but to hype the results more, provide better pointers to where they're stated, and tweak the statements a bit so they're easier to get the gist of if someone reads only Section 1 and then flips ahead to Section 4. Does what I've done look reasonable?}

% % \mfc{Yes, I agree}  \mfc{though the 4th paragraph feels apologetic.}
